Federated Fog Computing for Remote Industry 4.0 Applications

Industry 4.0 operates based on IoT devices, sensors, and actuators, transforming the use of computing resources and software solutions in diverse sectors. Various Industry 4.0 latency-sensitive applications function based on machine learning to process sensor data for automation and other industrial activities. Sending sensor data to cloud systems is time consuming and detrimental to the latency constraints of the applications, thus, fog computing is often deployed. Executing these applications across heterogeneous fog systems demonstrates stochastic execution time behavior that affects the task completion time. We investigate and model various Industry 4.0 ML-based applications' stochastic executions and analyze them. Industries like oil and gas are prone to disasters requiring coordination of various latency-sensitive activities. Hence, fog computing resources can get oversubscribed due to the surge in the computing demands during a disaster. We propose federating nearby fog computing systems and forming a fog federation to make remote Industry 4.0 sites resilient against the surge in computing demands. We propose a statistical resource allocation method across fog federation for latency-sensitive tasks. Many of the modern Industry 4.0 applications operate based on a workflow of micro-services that are used alone within an industrial site. As such, industry 4.0 solutions need to be aware of applications' architecture, particularly monolithic vs. micro-service. Therefore, we propose a probability-based resource allocation method that can partition micro-service workflows across fog federation to meet their latency constraints. Another concern in Industry 4.0 is the data privacy of the federated fog. As such, we propose a solution based on federated learning to train industrial ML applications across federated fog systems without compromising the data confidentiality.

==> B-abstract.tex <==
Industry 4.0 operates based on IoT devices, sensors, and actuators, transforming the use of computing resources and software solutions in diverse sectors. Various Industry 4.0 latency-sensitive applications function based on machine learning and utilize the generated sensor data for automation and other industrial activities. Sending sensor data to cloud systems is time consuming and detrimental to the latency constraints of the applications. In this circumstance, fog computing can be used to support latency-sensitive applications. Executing these applications across heterogeneous fog systems demonstrates stochastic execution time behaviour that affects the task completion time. Hence, we investigate and model various Industry 4.0 ML-based applications' stochastic executions and introduce real-world execution time traces of Industry 4.0 applications.

Remote offshore industries like oil and gas are prone to disasters requiring the coordination of various latency-sensitive activities. Accordingly, their procured fog computing resources can get oversubscribed due to the surge in the computing demands during a disaster. Hence, in this dissertation, we propose federating nearby fog computing systems and forming a fog federation to make remote Industry 4.0 sites resilient against the surge in computing demands. We propose a statistical resource allocation method across fog federation for latency-sensitive tasks. 

Many of the modern Industry 4.0 applications operate based on a workflow of micro-services that are used alone within an industrial site. As such, industry 4.0 solutions need to be aware of applications' architecture, particularly monolithic vs. micro-service. Therefore, we propose a probability-based resource allocation method that can partition micro-service workflows across fog federation to meet their latency constraints. Another concern in Industry 4.0 is the data privacy of the federated fog. As such, we propose a solution based on federated learning to train industrial ML applications across federated fog systems without compromising the data confidentiality.


==> B-acknowledgement.tex <==
~
            I sincerely thank my supervisor, Dr. \Supervisor, for his constant encouragement and passion for computer science and, especially, for his guidance, support, and cooperation. Thanks to my dissertation committee, Dr. Xu Yuan, Dr. Li Chen, and Dr. Sheng Chen. Thanks to Sm Zobaed, Ali Mokhtari, Davood Ghatreh Samani, and Chavit Denninart for their assistance in the work of this dissertation. Finally, thanks go to the Center for Advanced Computer Studies and the Graduate School at the University of Louisiana at Lafayette for their support and guidance.


==> B-dedicatory.tex <==
\vspace*{\fill}
\begin{center}
\textit{
To my wife, Rezwana Mahjabeen, my daughter, Ruzainah Shehzeen Hussain, my parents, H.K.M. Altaf Hussain and Fariha Akhter, my Sister, Sabrina Shahreen Sarna, my brother, Shoumin Rafsun Hussain and to all my friends and loved ones. 
}
\end{center}
\vspace*{\fill}



==> F-abstract.tex <==
\setlinespacing{1}
 \begin{description}
    \setlength{\parsep}{-3pt}
    \setlength{\itemsep}{-1.7pt}
    \setlength{\parindent}{0pt}
    \setlength{\labelsep}{-5pt}
    \item Zobaed, Sm.$\ $ 
                Bachelor of Science in Computer Science and Engineering, Islamic University of Technology, 2015;
                Master of Science, University of Louisiana at Lafayette,
                2019;
                Doctor of Philosophy, University of Louisiana at Lafayette,
                2022
    \item Major:$\ $                  \Major
    \item Title of Dissertation:$\ $  \Title
    \item Dissertation Director:$\ $  \Supervisor
    \item Pages in Dissertation:$\ $  180;  Words in Abstract:$\ $  347 %% UL limit it to 350
 \end{description}
\setlinespacing{1}
 \begin{theabstract}
 	\indent
                With the  meteoric growth of technology, 
both individuals to organizations are widely adopting cloud services to mitigate the burdens of maintenance. Despite its scalability and ease of use, many potential cloud users who own sensitive data refrain from fully utilizing cloud services due to valid confidentiality concerns. Maintaining data confidentiality for data at rest and in transit has been widely explored but data remains vulnerable in the cloud while it is in use. This vulnerability is further elevated once the scope of computing spans across the edge-to-cloud continuum.  From the notion of safeguarding, confidential data needs to be encrypted while offloading from users' premises. Although adopting user-side encryption ensures data confidentiality, it limits the ability to data processing. Subsequently, we are limited to performing only low-level operations (\eg string pattern matching). Accordingly, the goal of this dissertation is to enable data confidentiality by adopting confidential computing across the continuum. Towards this goal, one approach we explore is to separate the intelligence aspect of data processing from the pattern-matching aspect. We present our approach to make confidential data clustering on the cloud, and then develop  confidential search service across edge-to-cloud for unstructured text data. Our proposed clustering solution named ClusPr, performs topic-based clustering for static and  dynamic datasets that imposes cluster coherency upto 30\%-to-60\% when compared with other encyption-based clustering techniques. Our trusted enterprise search service named SAED, provides context-aware and personalized semantic search over confidential data across the continuum. Evaluation results, verified by human users, demonstrates that SAED can improve
the relevancy of the retrieved search results by $\approx$ 24\% for plain-text and 75\% for encrypted  datasets. We realized that enabling confidential computing across edge-to-cloud requires major contribution from the edge tiers particularly to run multiple Deep Learning (DL) services concurrently. This raises memory contention on the edge tier. To resolve the contention, we propose Edge-MultiAI framework to manage NN models of DL applications such that it can meet the latency constraints of the DL applications without compromising inference accuracy. Our evaluation confirms that Edge-MultiAI can stimulate the degree of multi-tenancy by $2\times$ on the edge tier.


\end{theabstract}

